Online Estimation of the Koopman Operator Using Fourier Features

Transfer operators offer linear representations and global, physically meaningful features of nonlinear dynamical systems. Discovering transfer operators, such as the Koopman operator, require careful crafted dictionaries of observables, acting on states of the dynamical system. This is ad hoc and requires the full dataset for evaluation. In this paper, we offer an optimization scheme to allow joint learning of the observables and Koopman operator with online data. Our results show we are able to reconstruct the evolution and represent the global features of complex dynamical systems.

==> sections/misc.tex <==
A dynamical system can be represented by:
\begin{equation}
    \dot{x} = f(x) 
\end{equation}
The discrete version of this dynamical system can be represented as:
\begin{equation}
    x_{k+1} = f(x_k)
\end{equation}
x is a set of states, where x belongs to the state space S, where $S \subset R^n$, and f is a mapping of those states forward in time, i.e. from time step $k$ to time step $k+1$, or describe the evolution of those states. \\

In the context of dynamical systems, data collected about the system are considered as knowledge of some variables related to the state of the system. \textbf{Data are the evaluation of functions of the states.} These functions of the states are called observables. \textit{Note that the definition of observable seems to be different in various papers. There can also be confusion with the controls theory literature.} 

Observables can include the pressure at a given point, or velocity at a set of points. \textbf{Knowledge of the state, i.e. data collected, like the velocity fields,  determine the value of the observable}. Let us use $h$ to denote the the observable of this dynamical system.

We know that x belongs to $S$, where $S \subset R^n$. Then, the observable of this dynamical system is given by a real-valued function $h : S \rightarrow \mathbb{R}$. \textcolor{pink}{The collection of all these observables makes a linear vector space.} We are not limited to studying the evolution of one observable though. Note that we can monitor a collection of multiple observables. The collection of multiple observables forms a linear vector space. So, with each real-valued function $h$, we obtain one corresponding dimension for our linear vector space.  With each new observable, we have an additional dimension. All observables evolve linearly under the Koopman operator. However, the Koopman operator is typically infinite-dimensional. This makes studying dynamical systems difficult. To make it easier, there are `special' observables that are Koopman invariant. These observables are called eigenfunctions of the Koopman operator. They are special in that they can be decoupled from the rest of the  regular observables, and together, they span a Koopman invariant subspace. This then means that the Koopman operator acts on a finite dimension, rather than an infinite dimension.

I.e. we could have image data with images of $ m \times n$, and each pixel represents one state. The dimensionality of this entire vector space is $\mathbb{R}^{m \times n}$. We could also have, say 5 measurements being acquired at 5 stationary locations in a 2-D space, and the state of these measurements can be monitored over time. The sub-space of the vector of these 5 points lives in $\mathbb{R}^5$, while this could live in $\mathbb{R}^{m \times n}$, if we assume sparsity, or the measurements are zero.   
\begin{equation}
    y_k = h(x_k)
\end{equation}
Where a set of observables change with time. The Koopman operator propagates this set of observables forward in time
